Linear interpolation gives better gradients than Gaussian smoothing in derivative-free optimization

In this paper, we consider derivative free optimization problems, where the objective function is smooth but is computed with some amount of noise, the function evaluations are expensive and no derivative information is available. We are motivated by policy optimization problems in reinforcement learning that have recently become popular [Choromaski et al. 2018; Fazel et al. 2018; Salimans et al. 2016], and that can be formulated as derivative free optimization problems with the aforementioned characteristics. In each of these works some approximation of the gradient is constructed and a (stochastic) gradient method is applied. In [Salimans et al. 2016] the gradient information is aggregated along Gaussian directions, while in [Choromaski et al. 2018] it is computed along orthogonal direction. We provide a convergence rate analysis for a first-order line search method, similar to the ones used in the literature, and derive the conditions on the gradient approximations that ensure this convergence. We then demonstrate via rigorous analysis of the variance and by numerical comparisons on reinforcement learning tasks that the Gaussian sampling method used in [Salimans et al. 2016] is significantly inferior to the orthogonal sampling used in [Choromaski et al. 2018] as well as more general interpolation methods.

==> app_experiments.tex <==
In all RL experiments the blackbox function $f$ takes as input the parameters of the policy $\pi_{\theta}:\mathcal{S} \rightarrow \mathcal{A}$ which maps states to proposed actions. The output of $f$ is the total reward obtained by an agent applying that particular policy $\pi_{\theta}$ in the given environment.

To encode policies $\pi_{\theta}$, we used fully-connected feedforward neural networks with two hidden layers, each of $h=41$ neurons and with $\mathrm{tanh}$ nonlinearities. The matrices of connections were encoded by low-displacement rank neural networks (see: \cite{choro2}), as in several recent papers on applying orthogonal directions in gradient estimation for ES methods in reinforcement learning.
We did not apply any additional techniques such as state/reward renormalization, ranking or filtering, in order to solely focus on the evaluation of the presented proposals.

All experiments were run with hyperparameter $\sigma=0.1$. 
Experiments that did not apply line search were run with the use of $\mathrm{Adam}$ optimizer and $\alpha = 0.01$. For line search experiments, we were using adaptive $\alpha$ that was updated via Armijo condition with Armijo parameter $c_{1}=0.2$ and backtracking factor $\tau=0.3$.



Finally, in order to construct orthogonal samples, at each iteration we were conducting orthogonalization of random Gaussian matrices with entries taken independently at random from $\mathcal{N}(0,1)$ via Gram-Schmidt procedure (see: \cite{choro2}). Instead of the orthogonalization of Gaussian matrices, we could take advantage of constructions, where orthogonality is embedded into the structure (such as random Hadamard matrices from \cite{choro2}), introducing extra bias but proven to work well in practice. However in all conducted experiments that was not necessary.

For each environment and each method we run $k=3$ experiments corresponding to different random seeds.

==> app_theory.tex <==
%In this section, we first restate the Assumptions that are used in the analysis (Sections \ref{sec:conv_analysis} and \ref{sec:grad_approx}). We them prove all the results that appear in the main paper (Lemmas \ref{lem.1} and \ref{lemma:bnd_var}; Theorems \ref{thm.conv}, \ref{thm.str}, \ref{thm.nonconvex} and \ref{lem:prob_bnd_smoothed}).
%
%\subsection{Assumptions}
%
%\begin{customassum}{\ref{assum.func_bnd}} \textbf{(Boundedness of Noise in the Function)} There is a constant $\epsilon_f \geq 0$ such that $ | f(x) - \phi(x)| = |e(x)| \leq \epsilon_f$ for all $x \in \mathbb{R}^n$.
%\end{customassum}
%
%\begin{customassum}{\ref{assum.lip_grad}} \textbf{(Lipschitz Continuity of the Gradients of $\pmb{\phi}$)} The function $\phi$ is continuously differentiable, and the gradients of $\phi$ are $L$-Lipschitz continuous for all $x \in \mathbb{R}^n$.
%\end{customassum}
%
%\begin{customassum}{\ref{assum.conv}} \textbf{(Convexity and bounded level sets of $\pmb{\phi}$)}  The function $\phi$ is convex and has bounded level sets, i.e., 
%\begin{align*}
%	\|x - x^\star\| \leq D, \quad \text{for all $x$ with } \ f(x) \leq f(x_0),	
%\end{align*}
%where $x^\star$ is a global minimizer of $\phi$. Let $\phi^\star = \phi(x^\star)$.
%\end{customassum}
%
%\begin{customassum}{\ref{assum.str_conv}} \textbf{(Strong Convexity of $\pmb{\phi}$)}  There exist a positive constant $\mu$ such that, for all $x,y \in \mathbb{R}^n$,
%\begin{align*}
%	\phi(y) \geq \phi(x) + \nabla \phi(x)^T (y-x) + \frac{\mu}{2} \| x - y \|^2.
%\end{align*}
%Let $\phi^\star = \phi(x^\star)$, where $x^\star$ is the minimizer of $\phi$.
%\end{customassum}
%
%\begin{customassum}{\ref{assum.lower_bnd}} \textbf{(Lower Bound on $\pmb{\phi}$)} The function $\phi$ is bounded below by a scalar $\hat{\phi}$.
%\end{customassum}
%
%\begin{customassum}{\ref{assum.lip_cont}}  \textbf{(Lipschitz Continuity of $\pmb{f}$)} The function $f$ is $L_f$-Lipschitz continuous  for all $x \in \mathbb{R}^n$.
%\end{customassum}
%
%\subsection{Proof of Lemma \ref{lem.1}}
%
%\begin{customlemma}{\ref{lem.1}} Let Assumptions \ref{assum.func_bnd} and \ref{assum.lip_grad} hold. If 
%\begin{align}		%\label{eq.alpha_bar}
%	\alpha_k \leq \bar{\alpha} = \frac{2(1-2\theta - c_1(1-\theta)}{L(1-\theta)}.
%\end{align}
%for $k=0,1,\dots$, and \eqref{eq.normcond} holds, then the relaxed Armijo condition \eqref{eq.rel_Arm} is satisfied. Moreover, for $k=0,1,\dots$
%\begin{align}		%\label{eq.decrease_phi}
%	\phi(x_{k+1}) \leq \phi(x_k) - c_1 \tau \bar{\alpha} (1-\theta)^2 \| \phi(x_k)\|^2 + 4 \epsilon_f.
%\end{align}
%\end{customlemma}
%
%\begin{proof} Since $\phi$ satisfies \ref{assum.lip_grad} and \eqref{eq.normcond} holds, we have
%\begin{align*}
%	\phi(x_k - \alpha_k g(x_k)) & \leq \phi(x_k) - \alpha_k g(x_k)^T \nabla \phi (x_k) + \frac{\alpha_k^2 L}{2} \| g(x_k)\|^2\\
%			& = \phi(x_k) - \alpha_k g(x_k)^T (\nabla \phi (x_k) - g(x_k)) - \left[1 -\frac{\alpha_k^2 L}{2}\right] \| g(x_k)\|^2\\
%			& \leq \phi(x_k) + \alpha_k \| g(x_k)\| \|\nabla \phi (x_k) - g(x_k)\| - \left[1 -\frac{\alpha_k^2 L}{2}\right] \| g(x_k)\|^2\\
%			& \leq \phi(x_k) + \frac{\alpha_k \theta}{1 - \theta }\| g(x_k)\|^2 - \left[1 -\frac{\alpha_k^2 L}{2}\right] \| g(x_k)\|^2\\
%			& \leq \phi(x_k) - \left[\frac{1-2\theta}{1-\theta} -\frac{\alpha_k^2 L}{2}\right] \| g(x_k)\|^2.
%\end{align*}
%By Assumption \ref{assum.func_bnd}, we have
%\begin{align*}
%	f(x_k - \alpha_k g(x_k)) \leq f(x_k) - \left[\frac{1-2\theta}{1-\theta} -\frac{\alpha_k^2 L}{2}\right] \| g(x_k)\|^2 + 2 \epsilon_f.
%\end{align*}
%From this we conclude that \eqref{eq.rel_Arm} holds whenever 
%\begin{align*}
%	f(x_k) - \left[\frac{1-2\theta}{1-\theta} -\frac{\alpha_k^2 L}{2}\right] \| g(x_k)\|^2 + 2 \epsilon_f \leq f(x_k) - c_1 \alpha_k \| g(x_k) \|^2 + 2\epsilon_f,
%\end{align*}
%which is equivalent to \eqref{eq.alpha_bar}.
%
%We have shown that when $\alpha_k \leq \bar{\alpha}$ the relaxed Armijo condition is \eqref{eq.rel_Arm} is satisfied. Since we find $\alpha_k$ using a constant backtracking factor of $\tau <1$, we have that $\alpha_k > \tau \bar{\alpha}$. Therefore, using Assumption \eqref{assum.func_bnd}, we have
%\begin{align*}
%	\phi(x_{k+1}) &\leq \phi(x_k) - c_1 \alpha_k \| g(x_k) \|^2 + 4\epsilon_f \\
%				& \leq \phi(x_k) - c_1 \tau \bar{\alpha} (1-\theta)^2 \| \nabla \phi(x_k) \|^2 + 4\epsilon_f,
%\end{align*}
%which completes the proof.
%\end{proof}
%
%\subsection{Proof of Theorem \ref{thm.conv}}
%\begin{customthm}{\ref{thm.conv}} Suppose that Assumptions \ref{assum.func_bnd}, \ref{assum.lip_grad} and \ref{assum.conv} hold. Let $\{ x_k \}$ be the iterates  generated by \eqref{eq.iteration}, where  $\alpha_k$ satisfies the relaxed Armijo condition \eqref{eq.rel_Arm}. Then, for $k=0,1,\dots$, 
%\begin{align}	\label{eq.convex}
%	\phi(x_{k}) - \phi^\star \leq \max \left\{ \frac{D^2}{k(1-\gamma)\eta}, \frac{2D \sqrt{\epsilon_f}}{\sqrt{\gamma \eta}}+4\epsilon_f\right\}, 
%\end{align}
%where $\eta = c_1 \tau \bar{\alpha}(1-\theta)^2$, and $\bar{\alpha}$ is given in \eqref{eq.alpha_bar}.
%\end{customthm}
%
%\begin{proof} By Assumption \ref{assum.conv}, we have
%\begin{align}	\label{eq.convex_D}
%	\phi(x_k) - \phi^\star \leq \nabla \phi(x_k)^T (x_k - x^\star) \leq \| \nabla \phi(x_k)\| \| x_k - x^\star \| \leq D \| \nabla \phi(x_k)\|.
%\end{align}
%Let $z_k = \phi(x_k) - \phi^\star$; by \eqref{eq.decrease_phi} and \eqref{eq.convex_D} we have,
%\begin{align*}
%	z_{k} - z_{k+1} \geq \frac{c_1 \tau \bar{\alpha} (1-\theta)^2 z_k^2}{D^2} - 4\epsilon_f.
%\end{align*}
%We thus have,
%\begin{align}	\label{eq.convex1}
%	\frac{1}{z_{k+1}} - 	\frac{1}{z_{k}} = \frac{z_k - z_{k+1}}{z_{k+1} z_k } \geq \frac{z_k - z_{k+1}}{ z_k^2 } \geq \frac{c_1 \tau \bar{\alpha} (1-\theta)^2 }{D^2} - \frac{4\epsilon_f}{z_k^2}.
%\end{align}
%We now consider two regimes: $(i)$ $z_i> \frac{2D \sqrt{\epsilon_f}}{\sqrt{\gamma c_1 \tau \bar{\alpha}}(1-\theta)}$, $\forall 0\leq i\leq k-1$ and $(ii)$ $z_i \leq \frac{2D \sqrt{\epsilon_f}}{\sqrt{\gamma c_1 \tau \bar{\alpha}}(1-\theta)}$, for some $0\leq i\leq k-1$,  where $\gamma \in (0,1)$. In the former case, the optimality gap is large compared to the noise, and thus by \eqref{eq.convex1} we have  $\forall 0\leq i\leq k$
%\begin{align}	\label{eq.convex2}
%	\frac{1}{z_{i+1}} - 	\frac{1}{z_{i}} \geq (1-\gamma) \frac{c_1 \tau \bar{\alpha} (1-\theta)^2 }{D^2}.
%\end{align}
%By aggregating this bounds for all  $\forall 0\leq i\leq k-1$ formula recursively, we obtain
%\begin{align}	\label{eq.convex3}
%	\frac{1}{z_{k}} \geq \frac{1}{z_{0}} + k(1-\gamma) \frac{c_1 \tau \bar{\alpha} (1-\theta)^2 }{D^2} \geq k(1-\gamma) \frac{c_1 \tau \bar{\alpha} (1-\theta)^2 }{D^2},
%\end{align}
%which yields the first part of the result in \eqref{eq.convex}. The second part of the result is obtained using three facts: the fact that there exists $i<k$ such 
%that $z_i\leq \frac{2D \sqrt{\epsilon_f}}{\sqrt{\gamma c_1 \tau \bar{\alpha}}(1-\theta)}$, the fact that for all $i$ $z_{i+1}-z_i\leq 4 \epsilon_f$ and for all
%$i$ such that $z_i> \frac{2D \sqrt{\epsilon_f}}{\sqrt{\gamma c_1 \tau \bar{\alpha}}(1-\theta)}$, $z_{i+1}-z_i\leq 0$. 
%\end{proof}
%
%\subsection{Proof of Theorem \ref{thm.str}}
%\begin{customthm}{\ref{thm.str}} Suppose that Assumptions \ref{assum.func_bnd}, \ref{assum.lip_grad} and \ref{assum.str_conv} hold. Let $\{ x_k \}$ be the iterates  generated by \eqref{eq.iteration}, where  $\alpha_k$ satisfies the relaxed Armijo condition \eqref{eq.rel_Arm}. Then, for $k=0,1,\dots$, 
%\begin{align}	\label{eq.strong1}
%	\phi(x_{k}) - \left[\phi^\star + \frac{4\epsilon_f}{1-\rho}\right]\leq \rho^k \left(\phi(x_0) -\left[\phi^\star + \frac{4\epsilon_f}{1-\rho}\right]\right), 
%\end{align}
%where $\rho = 1 - 2 \mu c_1 \tau \bar{\alpha}(1-\theta)^2$, and $\bar{\alpha}$ is given in \eqref{eq.alpha_bar}.
%\end{customthm}
%
%\begin{proof} Starting with \eqref{eq.decrease_phi}, by strong convexity we have $\| \nabla \phi (x_k)\|^2 \geq 2 \mu (\phi(x_k) - \phi^\star)$, thus
%\begin{align*}
%	\phi(x_{k+1}) - \phi^\star &\leq \phi(x_k) - \phi^\star - 2\mu c_1 \tau \bar{\alpha} (1-\theta)^2 (\phi(x_k) - \phi^\star) + 4 \epsilon_f\\
%		& = \rho(\phi(x_k) - \phi^\star) + 4 \epsilon_f.
%\end{align*}
%Subtracting $\frac{4 \epsilon_f}{1 - \rho}$ from both sides, 
%\begin{align*}
%	\phi(x_{k+1}) - \phi^\star - \frac{4 \epsilon_f}{1 - \rho} &\leq  \rho(\phi(x_k) - \phi^\star) + 4 \epsilon_f - \frac{4 \epsilon_f}{1 - \rho}\\
%			& = \rho(\phi(x_k) - \phi^\star) + \frac{(1- \rho)4 \epsilon_f - 4 \epsilon_f}{1 - \rho}\\
%			& = \rho(\phi(x_k) - \phi^\star) - \frac{\rho4 \epsilon_f}{1 - \rho}\\
%			& = \rho \left(\phi(x_k) - \phi^\star - \frac{4 \epsilon_f}{1 - \rho} \right).
%\end{align*}
%Recursive application of the above yields the desired result.
%\end{proof}
%
%\subsection{Proof of Theorem \ref{thm.nonconvex}}
%\begin{customthm}{\ref{thm.nonconvex}} Suppose that Assumptions \ref{assum.func_bnd}, \ref{assum.lip_grad} and \ref{assum.lower_bnd} hold. Let $\{ x_k \}$ be the iterates  generated by \eqref{eq.iteration}, where $\alpha_k$ satisfies the relaxed Armijo condition \eqref{eq.rel_Arm}. Then, for any $T\geq 1$,
%\begin{align*}
%	\frac{1}{T} \sum_{k=0}^{T-1} \| \nabla \phi(x_k)\|^2 &\leq \frac{\phi(x_0) - \hat{\phi}}{\eta T} + \frac{4 \epsilon_f}{\eta}\\
%			& \xrightarrow[]{T\rightarrow \infty} \frac{4 \epsilon_f}{\eta}.
%\end{align*}
%where $\eta =  c_1 \tau \bar{\alpha}(1-\theta)^2$, and $\bar{\alpha}$ is given in \eqref{eq.alpha_bar}.
%\end{customthm}
%
%\begin{proof} By \eqref{eq.decrease_phi}, we have
%\begin{align*}
%	\phi(x_{k+1}) \leq \phi(x_k) - c_1 \tau \bar{\alpha} (1-\theta)^2 \| \phi(x_k)\|^2 + 4 \epsilon_f,
%\end{align*}
%and thus
%\begin{align*}
%	\| \phi(x_k)\|^2 \leq \frac{\phi(x_k) - \phi(x_{k+1})}{c_1 \tau \bar{\alpha}(1-\theta)^2} + \frac{4 \epsilon_f}{c_1 \tau \bar{\alpha}(1-\theta)^2}
%\end{align*}
%Summing over the first $T-1$ iterations, 
%\begin{align*}
%	\sum_{k=0}^{T-1} \| \phi(x_k)\|^2 &\leq \sum_{k=0}^{T-1} \frac{\phi(x_k) - \phi(x_{k+1})}{c_1 \tau \bar{\alpha}(1-\theta)^2} + \sum_{k=0}^{T-1}\frac{4 \epsilon_f}{c_1 \tau \bar{\alpha}(1-\theta)^2}\\
%			& \leq \frac{\phi(x_0) - \hat{\phi}}{c_1 \tau \bar{\alpha}(1-\theta)^2} + \frac{4 \epsilon_fT}{c_1 \tau \bar{\alpha}(1-\theta)^2},
%\end{align*}
%where $\phi(x_0) - \hat{\phi} \geq \phi(x_0) - \phi(x_T)$. Averaging over the first $T-1$ iterations yields the desired result.
%\end{proof}
%
%\subsection{Proof of Theorem \ref{thm:bnd_linmod}}
%\begin{customthm}{\ref{thm:bnd_linmod}} Let $\mathcal{X}=\{x,x+\sigma u_1,\dots,x+\sigma u_n \}$ be set of interpolation points such that $\max_i\|u_i\|\leq 1$  and that 
%$Q_{\cal X}$ is nonsingular. Assume that $f(x)=\phi(x)+\epsilon(x)$, where $\phi(x)$ satisfies Assumption \ref{assum.lip_grad} and $\epsilon(x)\leq \epsilon_f$ for all $x$. Then, 
%\begin{align}
%	\|g({x}) - \nabla \phi(x)\| \leq \frac{\| Q_{\cal X}^{-1}\|_2\sqrt{n}\sigma L}{2} +\frac{2\| Q_{\cal X}^{-1}\|_2\sqrt{n}\epsilon_f}{\sigma}.
%\end{align}
%\end{customthm}
%
%\begin{proof}
%From the interpolation conditions and the mean value theorem $\forall i=1, \ldots, n$ we have 
%\begin{align}
%\sigma g(x)^T u_i &=f(x+\sigma u_i)-f(x)=\phi(x+\sigma u_i)-\phi(x)+\epsilon(x+\sigma u_i)-\epsilon(x)\\
%&=\int_{0}^t\sigma u_i^T\nabla \phi(x+t\sigma u_i)dt+\epsilon(x+\sigma u_i)-\epsilon(x).
%\end{align}
%From the $L$-smoothness of $\phi(\cdot)$ and the bound on $\epsilon(\cdot)$ we have 
%\begin{align}
%\sigma |(g(x)-\nabla \phi(x))^Tu_i| \leq  \frac {L\sigma^2 \|u_i\|^2}{2}+2\epsilon_f, \quad \forall i=1, \ldots, n
%\end{align}
%which in turn implies 
%\begin{align}
% \| Q_{\cal X}(g(x)-\nabla \phi(x))\| \leq  \frac {L\sigma \sqrt{n} }{2}+\frac{2 \sqrt{n} \epsilon_f}{\sigma},
%\end{align}
%and the theorem statement follows. 
%\end{proof}
%
%\subsection{Proof of Lemma \ref{lemma:bnd_var} and Theorem \ref{lem:prob_bnd_smoothed} }
%First we state some properties of normally distributed multivariate random variable $u \in \mathbb{R}^n$. 
%\begin{align}\label{eq:mvn}
%	&\mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[ u u^T \right]= I \nonumber\\
%		&\mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[ (u^Tu) u u^T \right]= (n+2)I \nonumber\\
%	&\mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[(a^T u)^2 u u^T \right]= a^T a I + 2 a a^T \nonumber\\
%	&\mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[a^T u \cdot u^T u \cdot u u^T \right]= 0_{n\times n} \\
%	&\mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[(u^T u)^2 u u^T \right]= (n+2)(n+4) I \nonumber\\
%         &\mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[a^T u \|u\|^3 \right]= 0,\nonumber\\
%	&\mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[(u^T u)^3 u u^T \right]= (n+2)(n+4)(n+8) I,\nonumber
%\end{align}
%where $a$ is any vector in $\mathbb{R}^n$ independent from $u$. We now provide bounds for the variance of GSG. 
%
%\begin{customlemma}{\ref{lemma:bnd_var}}
%Under Assumption  \ref{assum.lip_cont}, if $g(x)$ is calculated by \eqref{eq:GSG}, then, for all $x \in \mathbb{R}^n$,
%\begin{align*}	%\label{eq:var1_gauss}
%	\Var{g(x)} \preceq \kappa(x) I, \ \ \text{where} \ \ \kappa(x) = \frac{8 \|\nabla \phi(x)\|^2 +  L_f^2 n (n+2)(n+4)/\sigma^2+8(n+2)L_f^2n+16nL_f^2}{4N}.
%\end{align*} 
%
%%Alternatively, under Assumption  \ref{assum:lip_cont_hess}, if $g(x)$ is calculated by  \eqref{eq:cGSG}, then, for all $x \in \mathbb{R}^n$,
%%\begin{align*}	%\label{eq:var2_gauss}
%%	\Var{g(x)} \preceq \kappa(x) I, \ \ \text{where} \ \ \kappa(x) = \frac{108 \|\nabla f(x)\|^2 + M^2 \sigma^4 (n+2)(n+4)(n+8)}{36N}.
%%\end{align*} 
%\end{customlemma}
%%\end{framed}
%
%\begin{proof} 
%By \eqref{eq:var GSG}, we have 
%\begin{align*}
%	\Var{g(x)} &= \frac{1}{N} \mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[\left(\frac{f(x+\sigma u) - f(x)}{\sigma} \right)^2 u u^T \right ]- \frac{1}{N} \nabla \phi(x) \nabla \phi(x)^T \\
%	&\preceq \frac{1}{N \sigma^2} \mathbb{E}_{u \sim \mathcal{N}({0},I)} \left[\left( \nabla \phi(x)^T \sigma u + \frac{1}{2}L \sigma^2 u^T u+2\epsilon_f\right)^2 u u^T   \right]- \frac{1}{N} \nabla \phi(x) \nabla \phi(x)^T\\
%	&= \frac{1}{N \sigma^2} \mathbb{E}_{u \sim \mathcal{N}({0},I)} \Big[ \sigma^2 (\nabla \phi(x)^T u)^2 u u^T + L \sigma^3 (\nabla \phi(x)^T u) ( u^T u )u u^T  + \frac{1}{4} L^2 \sigma^4 (u^T u)^2 u u^T\\
%	&\quad   +4 \epsilon_f\sigma (\nabla \phi(x)^T u)uu^T + 2\epsilon_f L \sigma^2 (u^T u)uu^T +4\epsilon^2_f uu^T \Big] - \frac{1}{N} \nabla \phi(x) \nabla \phi(x)^T \\
%	&\stackrel{\mathclap{\mathrm{\eqref{eq:mvn}}}}{=} \frac{1}{N } \left( \nabla \phi(x)^T \nabla \phi(x) I + 2 \nabla \phi(x) \nabla \phi(x)^T\right) - \frac{1}{N} \nabla \phi(x) \nabla \phi(x)^T \\ &
%	+ \quad \frac{1}{\sigma^2N }\left( L \sigma^3 \cdot 0 + \frac{1}{4} L^2 \sigma^4 (n+2)(n+4)I +4 \epsilon_f\sigma\cdot 0+2(n+2)\epsilon_fL\sigma^2I+4\epsilon^2_fI\right)  \\
%	&\preceq \frac{ 8 \|\nabla \phi(x)\|^2 +   (n+2)(n+4)L^2\sigma^2 +8(n+2)\epsilon_fL}{4N}  I+\frac{4\epsilon^2_f}{\sigma^2N}I,
%\end{align*}
%where the first inequality comes from the Lipschitz continuity of the gradient of $\phi(x)$ and the bound  $|f(x)-\phi(x)|\leq \epsilon_f$
% and the last inequality is due to $\nabla \phi(x) \nabla \phi(x)^T \preceq \nabla \phi(x)^T \nabla \phi(x) I$. 
%
%Finally, we recall that for our choice of $\phi$, $L=\sqrt{n}L_f/\sigma$ and  $\epsilon_f=\sqrt{n}L_f\sigma$. Substituting these expressions in the above yields the desired result. 
%\end{proof}
%
%\begin{customthm}{\ref{lem:prob_bnd_smoothed}}
%Let $\phi$ be a Gaussian smoothed approximation of $f$ \eqref{eq: ES obj}. Under Assumption  \ref{assum.lip_cont}, if $g(x)$ is  calculated via \eqref{eq:GSG} with sample size
%\begin{align*}
%	N \ge \frac{2n \|\nabla \phi(x)\|^2}{\delta r^2} +\frac{L_f^2 n (n+2)(n+4)+8n(n+2)L_f^2+16nL_f^2}{4\delta r^2},
%\end{align*}
%then, for all $x \in \mathbb{R}^n$, $\|g(x) - \nabla \phi(x)\| \le r$ holds with probability at least $1 - \delta$, for any $r>0$ and $0< \delta<1$. 
%\end{customthm}
%%\end{framed}
%
%\begin{proof}
%By Chebyshev's inequality, for any $r > 0$, we have
%\begin{align*}
%\mathbb{P}\left\{\sqrt{(g(x) - \nabla \phi(x))^T \Var{g(x)}^{-1} (g(x) - \nabla \phi(x))} > r \right\} 
%&\le \frac{n}{r^2}. 
%\end{align*}
%Since $\Var{g(x)} \preceq \kappa I$, we have $\Var{g(x)}^{-1} \succeq \kappa^{-1} I$ and 
%\[ \sqrt{(g(x) - \nabla \phi(x))^T \Var{g(x)}^{-1} (g(x) - \nabla \phi(x))} \ge \kappa^{-\frac{1}{2}} \|g(x) - \nabla \phi(x)\|.
%\]
%Therefore, we have, 
%\begin{align*}
%\mathbb{P}\left\{\kappa^{-\frac{1}{2}} \|g(x) - \nabla \phi(x)\| > r \right\} \le \frac{n}{r^2}  \ \ \Longrightarrow \ \
%\mathbb{P}\left\{ \|g(x) - \nabla \phi(x)\| > r \right\} \le \frac{\kappa n}{r^2}. 
%\end{align*}
%By Lemma \ref{lemma:bnd_var}, for GSG we have
%\begin{align*}
%	\mathbb{P}\left\{ \|g(x) - \nabla \phi(x)\| > r \right\} &\le \frac{2n \|\nabla \phi(x)\|^2}{N r^2} +
%	\frac{L_f^2 n (n+2)(n+4)+8n(n+2)L_f^2+16nL_f^2}{4N r^2}.
%\end{align*} 
%Thus when 
%$$
%N \ge \frac{2n \|\nabla \phi(x)\|^2}{\delta r^2} + \frac{L_f^2 n (n+2)(n+4)+8n(n+2)L_f^2+16nL_f^2}{4\delta r^2},
%$$
% we have $\mathbb{P}\left\{ \|g(x) - \nabla \phi(x)\| > r  \right\} \le \delta$. 
%
%
%\end{proof}
%

